Towards a Digital Highway Code using Formal Modelling and Verification of Timed Automata

One of the challenges in designing safe, reliable and trustworthy Autonomous Vehicles (AVs) is to ensure that the AVs abide by traffic rules. For this, the AVs need to be able to understand and reason about traffic rules. In previous work, we introduce the spatial traffic logic USL-TR to allow for the unambiguous, machine-readable, formalisation of traffic rules. This is only the first step towards autonomous traffic agents that verifiably follow traffic rules. In this research preview, we focus on two further steps: a) retrieving behaviour diagrams directly from traffic rules and b) converting the behaviour diagrams into timed automata that are using formulae of USL-TR in guards and invariants. With this, we have a formal representation for traffic rules and can move towards the establishment of a Digital Highway Code. We briefly envision further steps which include adding environment and agent models to the timed automata to finally implement and verify these traffic rule models using a selection of formal verification tools.

==> eptcsdata.tex <==
\providecommand{\firstpage}{77}
\providecommand{\publicationstatus}{M. Luckcuck and M. Farrell; M. Autili, L. Berardinelli,\\ A. Bucaioni and C. Pompilio (Eds.):\\
Formal Methods for Autonomous Systems and \\
Automated and verifiable Software sYstem DEvelopment \\
EPTCS 371, 2022, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.371.6}{10.4204/EPTCS.371.6}}
\pdfoutput=1

